Random Sampling for Group-By Queries

Random sampling has been widely used in approximate query processing on large databases, due to its potential to significantly reduce resource usage and response times, at the cost of a small approximation error. We consider random sampling for answering the ubiquitous class of group-by queries, which first group data according to one or more attributes, and then aggregate within each group after filtering through a predicate. The challenge with group-by queries is that a sampling method cannot focus on optimizing the quality of a single answer (e.g. the mean of selected data), but must simultaneously optimize the quality of a set of answers (one per group). We present CVOPT, a query- and data-driven sampling framework for a set of group-by queries. To evaluate the quality of a sample, CVOPT defines a metric based on the norm (e.g. $\ell_2$ or $\ell_\infty$) of the coefficients of variation (CVs) of different answers, and constructs a stratified sample that provably optimizes the metric. CVOPT can handle group-by queries on data where groups have vastly different statistical characteristics, such as frequencies, means, or variances. CVOPT jointly optimizes for multiple aggregations and multiple group-by clauses, and provides a way to prioritize specific groups or aggregates. It can be tuned to cases when partial information about a query workload is known, such as a data warehouse where queries are scheduled to run periodically. Our experimental results show that CVOPT outperforms current state-of-the-art on sample quality and estimation accuracy for group-by queries. On a set of queries on two real-world data sets, CVOPT yields relative errors that are 5x smaller than competing approaches, under the same space budget.

==> combination_sample.tex <==
%--------------------------------------------------------------
%\subsection{Combination Sample for Multiple Group-By Queries}
\subsection{Individual Stratification}
\label{sec:combine}
%--------------------------------------------------------------
The finest stratification discussed in Section~\ref{sec:finest} yields
a collection of strata that can always collectively serve a group-by
query whose grouping attributes is a subset of the attributes used for
the finest stratification. However, the number of strata in the
finest stratification may become close to or even larger than the memory
space $M$, making the idea of sampling over
the finest strata using the memory $M$ fail. In this section, we present an
alternative framework, named \emph{individual stratification}, for
sampling for group-by queries. Our presentation focuses on 
the case of multiple aggregates and multiple
group-bys (MAMG). Other scenarios (SASG, SAMG, MASG) will be
the special cases of MAMG.


%In Section~\ref{sec:sg}, we introduced algorithm to draw the optimal
%sampled table for a group-by query with the given sample space. 
%In this section, we consider multiple group-by queries. 
The idea is to consider each group-by query individually and 
sample each  group of each group-by query. However, the memory usage by
all the stratified samples of all group-by queries is constrained up
to 
$M$. We consider all the stratified random sampling over all groups of
all group-by queries collectively 
and have them all together into a 
optimization problem whose solution is the best memory
allocation size for each group of each group-by query. When answering
a group-by query, all stratified samples will be collectively and
carefully used in order to make full use of these samples.

%The insight is to use the combination of individual samples into one
%and use it to have better answer for each and every query. 
Suppose we have $m$ group-by queries $Q_1, Q_2, \ldots, Q_m$. Each
query aggregates a set of columns, denoted as $\mathcal{L}_i$. For
different $i$ and $j$, $\mathcal{L}_i$ and $\mathcal{L}_j$ may or may
not overlap with each other. Let $G_i$ denote the set of groups 
induced by query $Q_i$. 
%Section~\ref{sec:sasg} shows how to derive a
%sub-sample for each query, in which each sub-sample serves that query
%the best.


Consider a query $Q_i$, for each of its group $g \in G_i$ and each of
its aggregate columns $\ell \in \mathcal{L}_i$: let $\mu_{i,g,\ell}$
and $\sigma_{i,g,\ell}$ denote the mean and standard deviation of
values from the aggregate column $\ell$ among all elements belonging
to group $g$;
$\gamma_{i,g,\ell}=\frac{ \sigma_{i,g,\ell} }{ \mu_{i,g,\ell} }$, the
coefficient of variation; Let $n_{i,g}$ denote the size of the group.
Let $s_{i,g}$ denote that sample size we allocate for the group.  Note
that each sample is a whole row of the table.

We want
to decide each sample size $s_{i,g}$ such that the
estimates $y_{i,g,\ell}$ for
each $\mu_{i,g,\ell}$ is overall the best for all $i$ and $g$. 
Our goal is translated into minimizing 
the weighted $\ell_2$ norm of
$\{\cv{y_{i,g,\ell}} | i \in [1..m], j \in G_i, \ell \in \mathcal{L}_i \}$, i.e. our
optimization function is
\[
\sqrt{ \sum_{i=1}^{m} \sum_{g\in G_i}\sum_{\ell\in \mathcal{L}_i}
  w_{i,g,\ell}\cdot \left(\cv{y_{i,g,\ell}}\right)^2 }
\]
under the contraint that $\sum_{i=1}^{m} \sum_{g\in G_i} s_{i,g} = M$.

%------------------------
\begin{theorem}
\label{thm:combination}
The optimal assignment of sample space $M$ among all groups of all
queries is to assign to each group $g \in G_i$ of each $Q_i$, $i \in
[1\ldots k]$, 
the sample size 
$$
s_{i,g} = M \cdot \frac{\sqrt{\sum_{\ell\in
      \mathcal{L}_i}\left(w_{i,g,\ell}\cdot \gamma_{i,g,\ell}^2\right)}} 
{\sum_{j=1}^{m} \sum_{t\in G_j} \sqrt{\sum_{q\in
      \mathcal{L}_j}\left(w_{j,t,q} \cdot \gamma_{j,t,q}^2\right)}}
$$
\end{theorem}
%------------------------

%------------------------
\begin{proof}
  Because $y_{i,g,\ell}$ is an unbiased estimate, we have
  $\cv{y_{i,g,\ell}} = =\frac{\std{y_{i,g,\ell}}}{\mu_{i,g,\ell}}$,
  where $\std{y_{i,g,\ell}}$ and $\mu_{i,g,\ell}$ are the standard
  deviation and mean of the estimate $y_{i,g,\ell}$. By standard
  results on sample (e.g. see Theorem 2.2 in \cite{Coch77:book}), we
  have
  $\std{y_{i,g,\ell}} =
  \sqrt{\frac{\sigma_{i,g,\ell}^2(n_{i,g}-s_{i,g})}{n_{i,g} s_{i,g}}}$.
  Thus, it reduces to minimize

\[\sum_{i=1}^{m} \sum_{g\in G_i} \sum_{\ell \in \mathcal{L}_i} 
\frac{w_{i,g,\ell} \cdot \sigma_{i,g,\ell}^2(n_{i,g}-s_{i,g})} { n_{i,g} s_{i,g} \mu_{i,g,\ell}^2 } \] 

Since $n_{i,g}$, $\sigma_{i,g,\ell}$ and $\mu_{i,g,\ell}$  are fixed, this is equivalent to minimizing:
% --------------
$$
\sum_{i=1}^{m} \sum_{g\in G_i}\sum_{\ell\in\mathcal{L}_i}
\frac{w_{i,g,\ell}\cdot \sigma_{i,g,\ell}^2} {\mu_{i,g,\ell}^2} 
\frac{1}{s_{i,g}}
= \sum_{i=1}^{m} \sum_{g\in G_i}\frac{\sum_{\ell\in\mathcal{L}_i} \left(w_{i,g,\ell}\cdot\gamma_{i,g,\ell}^2\right)}{s_{i,g}}
$$
% --------------
subject to condition:
% --------------
$
\sum_{i=1}^{m} \sum_{g\in G_i} s_{i,g} = M.
$
% --------------
Using Lemma~\ref{lem:opt-helper}, we arrive that the optimal
sample size assignment $s_{i,g}$ for group $g$ of query $Q_i$ is proportional to
the square root of
$\sum_{\ell\in
      \mathcal{L}_i}(w_{i,g,\ell}\cdot\gamma_{i,g,\ell}^2)$.
%
%$$
%s_{i,g} = M \cdot \frac{\sqrt{\sum_{\ell\in
%     \mathcal{L}_i}\gamma_{i,g,\ell}^2}} 
%{\sum_{j=1}^{m} \sum_{t\in G_j} \sqrt{\sum_{q\in
%      \mathcal{L}_j}\gamma_{j,t,q}^2}}
%$$
\end{proof}
%------------------------

\subsubsection{A Unified Sample for MAMG}
Obviously, if we continue to draw $s_{i,g}$ random samples (denoted as
$S_{i,g}$) from each group $g\in G_i$ of each query $Q_i$, in the
resulting collection of stratified randome samples, many table rows
may be selected more than once with different probability. On the other
hand, we do not want to only use the samples $S_{i,*}$ to address the
query $Q_i$, because there are other available samples of the table
rows and having them included in the calculation can obviously improve
the accuracy of the estimate. In order to make full use of the full
memory space in address each query, we will draw and maintain a
unified collection of samples that will be used to serve all queries.

We first calculate the optimal sample size allocation $s_{i,g}$ for
each group $g\in G_j$ of each query $Q_i$, using the optimization
framework under the individual stratification.  Then, for each row $r$
that belongs to group $g$ of query $Q_i$, we assign the row $r$ a
sample rate $p_{r,i} = s_{i,g}/n_{i,g}$. Then,
let $p_r = 1- \prod_{i=1}^m (1-p_{r,i})$ 
%$p_r = \sum_{i=1}^m p_{r,i}$ 
be the probability of the row $r$ to be
included in the final sample. After the computation of $p_r$ for all
$r \in [1..n]$, we simply follow a Poisson random sampling~\cite{xxx} procedure
to draw a sample whose size is expected to be no more than $M$. Upon receiving any
group-by query, we will use the Poisson sample to address the query, where
the contribution of each selected  table row $r$ is augmented by a factor
%of $1/p_r$. {\color{red} (please double check its correctness.)}
%
%
%\bigskip 
%\bigskip 
%\bigskip 
%\bigskip 
%\todo{not sure the rest will still be needed ... }
%
%Having the sample space allocation $s_{ij}$ for each group $j$ of query $Q_i$, one can draw $m$ sub-samples. Then all the sub-samples are combined into a single sample table. Obviously the combination of sub-samples give us a better sample. To answer any query $Q_i$, we have a sample which is a super set of the sub-sample that we draw intently to answer that query. On the other hand, the combined sample leads to the nonuniform in the sample of each stratum we have. That is the records belong to that a same group are not uniformly selected, as they are in each sub-sample. We maintain the nonuniform sample by adding an extra column to the sampled table, named {\tt sample\_rate}. This attribute keeps the sample property of each record when it's selected. By that, we can have the unbiased estimations from the nonuniform stratified sampling. For example, when the sample is uniform with the selection probability $p$, the unbiased estimation of the sum is $S =\frac{1}{p} \sum_{x \in Sample} x$. The unbiased estimation of the sum from the nonuniform sample is $S = \sum_{x \in Sample} \frac{x}{p_x}$, where $p_x$ is the probability x was selected.
%
%Drawing $m$ sub-samples independently creates the overlapping among sub-samples, which leads to either duplication in the final sample, or wasting of sample space, depends on the combination procedure is concatenation or union. We address this issue by combining the \textit{sample allocations} then use the combined sample allocation to draw a single sample, instead of combining $m$ independent sub-samples.
%To do so, we first convert the sample size allocation into selection probability. Let $n_{i,j}$ is the size of the group $j = 1, 2, \ldots r_i$ of query $Q_i, i \in [1 \ldots m]$. By applying Poisson sampling~\cite{?} with selection probability:
%
%\[ p_{i,j} = \frac{ s_{i,j} }{ n_{i, j} } 
%= \frac{M \gamma_{i,j} } {n_{i,j} \sum_{k=1}^{m} \sum_{t=1}^{r_k} \gamma_{k,t}} \]
%
%That is, each record in the group have the same chance of $p_{i,j}$ to be selected into the sample, we expectedly have an sample of designed size $s_{i,j}$. While we have $m$ queries, a record $x$ belongs to $m$ different groups. Assuming their converted selection rate are $p_{1,x}, p_{2,x}, \ldots p_{m,x}$, the record is not selected into the combined sample only if it is not chosen into any sub-sample, which happens with probability $(1-p_{1,x})(1-p_{2,x}) \ldots (1-p_{m,x})$. In the other words, each record $x$ is selected with probability:
%\begin{equation}
%p_x = 1 - \prod_{i = 1}^{m} (1 - p_{i,x})
%\end{equation}
%where $p_{i,x}$ is the selection probability of the group that record $x$ belongs to, due to the query $Q_i, i \in 1 \ldots m$. 

%------------------------
\begin{algorithm}[t]
\small
\DontPrintSemicolon
\label{algo:combine}
\KwIn{Database Table $T$, group-by queries $Q_1, Q_2, \ldots Q_m$, space budget $M$.}
\KwOut{Stratified Random Sample $S$}

Let $\universeA_i(x)$ denote the group assignments of record $x \in T$, due to query $Q_i, i \in 1 \ldots m$. Let $r_i$ denote the number of distinct values of $\universeA_i$, and suppose the strata are numbered from $1$ till $r_i$\\

For each query $Q_i, i = 1 \ldots m$, and for each of its strata $j = 1\ldots r_i$, compute the coefficient of variation and number of all elements in stratum $j$, denoted as $\gamma_{i,j}$ and $n_{i,j}$ respectively.

$\gamma \gets \sum_{i=1}^m \sum_{j=1}^{r_i} \gamma_{i,j}$ \\

\textit{\# Poisson sampling}

\For{$x \in T$}
{
	\If {\tt Rand() < $1 - \prod_{i=1}^{m} \left( 1 - M \frac{\gamma_{i,\universeA_i(x)}}{n_{i,\universeA_i(x) \gamma}}  \right) $}
	{
		$S \gets S \cup \{x\}$
	}
}

\KwRet{$S$}
\caption{\combinesamg: An algorithm for computing a combined sample for multiple single-aggregate group-by queries}
\end{algorithm}
%------------------------


==> extension.tex <==
\section{Extension to Other Aggregates}
\label{sec:ext}
So far the discussion of our \cvopt framework is focused on group-by
queries for the mean estimate, but the \cvopt framework indeed can be
used for other aggregates as well. 
To use the \cvopt framework for an aggregate, all
we need is to: 1) have the per-group CV of the aggregate of interest well defined,
and 2) also ensure the aggegate's CV of a stratum $A$ can be obtained from
the CV of $A$'s
non-empty substrata $B$ and $C$, where $A=  B \cup C$ and $B\cap C = \emptyset$.
Example aggregates that can be handled by our \cvopt framework 
include the per-group sum, count, vairance,
median, etc. 
\todo{pls double check the above writing. Not so sure about the
  variance and median.}




==> metric.tex <==
\section{Single Aggregate Query with a Single Group-by}

We use stratified sampling to draw a bias sample from the full table. The stratification is based on group-by clause to minimize the missing groups in result. The research question: How do we allocate a given limited memory budget among strata (groups) to get the \textit{best} sample? We first define a measurement for evaluate the quality of sample for group-by query. Then we propose a allocation algorithm to divide a given memory budget to minimize the estimated error.

\subsection{Coefficient of Variation}
Let $\mu_i$ denote the mean of entire stratum $i$. The sample mean of a uniform random sample $S_i$ of size $s_i$ drawn
from stratum $i$ without replacement is
defined as: $\bar{\mu}_i = \frac{ \sum_{v \in S_i} } {s_i}$. 
We have $\bar{\mu_i}$ is an unbiased estimate of $\mu_i$, \ie $E(\bar{\mu_i})=\mu_i$. Even thought $\bar{\mu_i}$ is an ubniased estimate, the \textit{actual} value we get from sample is various due to the randomness of drawing samples.
Let $\cvn_i$ denote the standard deviation of $\bar{\mu_i}$. 
By Theorem 2.2 in \cite{Coch77:book}, we have:

\begin{equation}
\cvn_i = \sqrt{\frac{\sigma_i^2(n_i-s_i)}{n_i s_i}},
\end{equation}
where $\sigma_i$ and $n_i$ denote the standard deviation and the size of the entire stratum $i$.
%
$d_i$ measures the \textit{confidence} of the estimation $\bar{\mu_i}$. Intuitively, the smaller $d_i$, the more confident estimate $\bar{\mu_i}$. We say a sample $S_i$ that has smaller $d_i$ is a better sample. As seen, the confidence of the estimate is inverse ratio with size of the sample, $s_i$. Naturally, the larger sample leads to a better estimation. Especially, when we keep all the records of stratum $i$ as its sample, $s_i = n_i$, we have $d_i = 0$, \ie the answer from \textit{sample} is the \textit{exact answer}.

Standard deviation $d_i$ is a good measurement of the sample quality for stratum $i$, however it is incomparable between strata, since standard deviation depends on of the magnitude of the values. \eg Consider samples from two strata $i$ and $j$ with corresponding estimated means $\bar{\mu}_i=1000, \bar{\mu}_j=100$ and standard deviations $d_i=d_j=10$. Those two estimates have equal standard deviation but their qualities are different. Assume that both two strata follow normal distribution, with high probability ($>96\%$ chances) the truth value of the mean $\mu_i$ is between $\left[{950; 1050}\right]$ and $\mu_j$ is between $\left[50; 150\right]$. In other words, $\mu_i = \bar{\mu}_i \pm 5\%$ meanwhile $\mu_j = \bar{\mu}_j \pm 50\%$. 

We introduce an error metric for per-stratum query over stratum $i$ to normalize the magnitude of the standard deviation:
\begin{equation}
\epsilon_i = \frac{\cvn_i}{\mu_i}
\end{equation}


\todo{(1) Is it better to explain why the above new error metric solves
  the concern/problem from the discussion in the above example ? (2) The
  basic/intuitive idea is to ensure the ``relative errors'' over all
  strata to be the same (or close?). (3) If we want to intentionally give extra favors
to some strata, it might be done by adding some multiplicative ``weight''
constant to each $\epsilon_i$.}

%\bigskip 
%\noindent
%The optimization problem is to minimize the average error:
%\begin{eqnarray}
%\epsilon_{L_1} = \frac{1}{r} \sum_{i=1}^{r}\epsilon_i
% = \frac{1}{r}  \sum_{i=1}^r \frac{d_i}{\mu_i}
% =  \frac{1}{r}  \sum_{i=1}^r \sqrt{\frac{\sigma_i^2(n_i-s_i)}{n_i
%  \mu_i^2 s_i}}
% =  \frac{1}{r}  \sum_{i=1}^r \sqrt{
%\frac{\sigma_i^2}{\mu_i^2 s_i}
%-\frac{\sigma_i^2}{n_i \mu_i^2}
%}
%\end{eqnarray}
%subject to
%\begin{equation}
%\sum_{i=1}^{r} s_i = M,
%\end{equation}
%where $M$ is the total sample size or memory budget.
%
%
%\bigskip 
%\bigskip 
%It seems easier to handle the math, if we choose to minimize  the other error
%metric: 
We use Euclidean norm of $\epsilon$ to measure over-all error of all $r$ strata:  
\begin{eqnarray}
\epsilon_{L_2} = \sqrt{\frac{1}{r} \sum_{i=1}^{r}\epsilon_i^2}
= \sqrt{\frac{1}{r}\sum_{i=1}^{r} \left(\frac{\sigma_i^2}{\mu_i^2 s_i}
-\frac{\sigma_i^2}{n_i \mu_i^2}\right)}
\label{eqn:eps2}
\end{eqnarray}

We aim to allocate the given sample space $M$ between $r$ strata, in which we minimize $\epsilon_{L_2}$. Because $r$, $\sigma_i$, $\mu_i$, and $n_i$ are all fixed, it is equivalent to minimizing:
\begin{eqnarray}
\sum_{i=1}^r \frac{\sigma_i^2}{\mu_i^2s_i}
= \sum_{i=1}^r \frac{\sigma_i^2/\mu_i^2}{s_i} \label{eqn:eps2-2}
\end{eqnarray}
subject to the condition:
\begin{equation}
\sum_{i=1}^{r} s_i = M
\end{equation}

\begin{theorem}
Optimal solution for Equation~\ref{eqn:eps2-2} is, for $i=1,2,\ldots, r$: 
$$s_i = M \frac{\sigma_i/\mu_i}{\sum_{j=1}^r \sigma_j/\mu_j}$$ 
\label{conj_optimal_allocate}
\end{theorem}

\begin{proof}
Denote functions $f(.),g(.)$ as:
$$f(s_1,s_2,...,s_r)=\sum_{i=1}^r \frac{\sigma_i^2/\mu_i^2}{s_i}$$
$$g(s_1,s_2,...,s_r)=\sum_{i=1}^{r} s_i - M$$
We want to minimize $f(.)$ with the constraint $g(.)=0$.
Using Lagrange multipliers, with Lagrange function is:
$$L(s_1,s_2,...,s_r,\lambda)=f(s_1,s_2,...,s_r) + \lambda g(s_1,s_2,...,s_r)=\sum_{i=1}^r \frac{\sigma_i^2/\mu_i^2}{s_i}+\lambda\left(\sum_{i=1}^{r} s_i - M\right)$$
we have, for $i=1,..,r$:
$$\frac{\partial L}{\partial s_i}=-\frac{\sigma_i^2/\mu_i^2}{s_i^2}+\lambda$$
Let $\frac{\partial L}{\partial s_i}=0\Rightarrow s_i=\frac{\sigma_i/\mu_i}{\sqrt{\lambda}}$; And let $g(.)=0$,
$$\sum_{i=1}^{r} s_i - M=0\Rightarrow M=\frac{1}{\sqrt{\lambda}}\sum_{i=1}^{r}\sigma_i/\mu_i\Rightarrow \frac{1}{\sqrt{\lambda}}=\frac{M}{\sum_{i=1}^{r}\sigma_i/\mu_i}$$
Thus,
$$s_i = M \frac{\sigma_i/\mu_i}{\sum_{j=1}^r \sigma_j/\mu_j}$$ 
\end{proof}

Theorem~\ref{conj_optimal_allocate} says, to gain the minimal over-all error $\epsilon_{L_2}$, we should allocate to each stratum $i$ the sample space proportioned to its standard deviation divided by its mean: $\sigma_i / \mu_i$. That is intuitive, since the strata with larger standard deviation, relatively to its mean, have the values spread widely, thus, they are harder to estimate. We give those strata more samples in order to have good quality estimations. Meanwhile, we make trade-off with other strata that have relatively smaller standard deviation, since their values are more concentrated, they requite fewer samples to gain the same level of confidence.

\todo{Shall we discuss here the consequence of this memory allocation
  policy in terms of the ``relative error''  for each stratum. For ex.,
  Will the relative errors of all strata be the same, or close, how
  close, etc ? }
\subsection{Bounded Strata}

\begin{algorithm}
\caption{Caption goes here...}
\label{alg_bounded_strata}

Algorithm goes here.
\end{algorithm}

Theorem~\ref{conj_optimal_allocate} shows that, the sample size of each stratum $i$ should be proportional to $\sigma_i/\mu_i$. Practically, underpopulated stratum may has size smaller than the ideal sample size, \eg $n_i < s_i$. We call those strata, whom size smaller than optimal sample size, are bounded strata. Intuitively, the sample should include all the records from bounded strata, \eg let $s_i = n_i$. That leads to a sub-optimal solution, since it violates the constrain $g(.) = 0$, \eg total sample space is less than the given memory budget.
\todo{cite Voila}

We address this sub-optimal issue by first select all records from
bounded strata and take them out of further consideration. Then, we
re-allocate the leftover space between those remaining strata. Note
that, in this second round of allocation, the bounded strata
phenomenon may appear again. Since the memory is relatively larger
than the first round, some strata among the remaining strata may
become bounded. Thus, we recursively apply the procedure until all the
strata are unbounded. Finally, we apply the last round of allocation
on those unbounded strata follow
Theorem~\ref{conj_optimal_allocate}. Algorithm~\ref{alg_bounded_strata}
shows detail of the algorithm to allocate the memory between
strata. \todo{This descirbed procedure needs a proof to show its optimality. Proof shall be
  similar to the one for VOILA but using the new error metric (Equation~\ref{eqn:eps2-2}).}


==> ptcds_query.tex <==
\section{TPC-DS Queries}
%--------------- TPCDS Query 2
\begin{query}[b]
\begin{lstlisting}[language=SQL]
WITH wscs AS (
  SELECT sold_date_sk,
         sales_price
  FROM (
    SELECT ws_sold_date_sk sold_date_sk,
           ws_ext_sales_price sales_price
    FROM web_sales
  ) x
  UNION ALL
  SELECT cs_sold_date_sk sold_date_sk,
         cs_ext_sales_price sales_price
  FROM catalog_sales
),
wswscs AS (
  SELECT d_week_seq,
    sum(CASE WHEN (d_day_name = 'Sunday')
        THEN sales_price ELSE NULL
        END) sun_sales,
    sum(CASE 
        WHEN (d_day_name = 'Monday')
          THEN sales_price
        ELSE NULL
        END) mon_sales,
    sum(CASE 
        WHEN (d_day_name = 'Tuesday')
          THEN sales_price
        ELSE NULL
        END) tue_sales,
    sum(CASE 
        WHEN (d_day_name = 'Wednesday')
          THEN sales_price
        ELSE NULL
        END) wed_sales,
    sum(CASE 
        WHEN (d_day_name = 'Thursday')
          THEN sales_price
        ELSE NULL
        END) thu_sales,
    sum(CASE 
        WHEN (d_day_name = 'Friday')
          THEN sales_price
        ELSE NULL
        END) fri_sales,
    sum(CASE 
        WHEN (d_day_name = 'Saturday')
          THEN sales_price
        ELSE NULL
        END) sat_sales
  FROM wscs,
    date_dim
  WHERE d_date_sk = sold_date_sk
  GROUP BY d_week_seq
  )
SELECT d_week_seq1,
  round(sun_sales1 / sun_sales2, 2),
  round(mon_sales1 / mon_sales2, 2),
  round(tue_sales1 / tue_sales2, 2),
  round(wed_sales1 / wed_sales2, 2),
  round(thu_sales1 / thu_sales2, 2),
  round(fri_sales1 / fri_sales2, 2),
  round(sat_sales1 / sat_sales2, 2)
FROM (
  SELECT wswscs.d_week_seq d_week_seq1,
    sun_sales sun_sales1,
    mon_sales mon_sales1,
    tue_sales tue_sales1,
    wed_sales wed_sales1,
    thu_sales thu_sales1,
    fri_sales fri_sales1,
    sat_sales sat_sales1
  FROM wswscs,
    date_dim
  WHERE date_dim.d_week_seq = wswscs.d_week_seq
    AND d_year = 2001
  ) y,
  (
    SELECT wswscs.d_week_seq d_week_seq2,
      sun_sales sun_sales2,
      mon_sales mon_sales2,
      tue_sales tue_sales2,
      wed_sales wed_sales2,
      thu_sales thu_sales2,
      fri_sales fri_sales2,
      sat_sales sat_sales2
    FROM wswscs,
      date_dim
    WHERE date_dim.d_week_seq = wswscs.d_week_seq
      AND d_year = 2001 + 1
    ) z
WHERE d_week_seq1 = d_week_seq2 - 53
ORDER BY d_week_seq1;
  -- end query 1 in stream 0 using template query2.tpl



\end{lstlisting}
\caption{TPC-DS Query 2}
\label{query:tpcds_02}
\end{query}
%---------------



==> streaming.tex <==
%-----------------------------
\section{Streaming}
\label{sec:stream}
%-----------------------------
We now consider the case, where new tuples of a database table
continues to arrive as a stream. We want to dynamically maintain an
SRS over the stream using limited memory space.  Over the evolving of
the stream, the sample size allocation for different groups changes,
so does the actual sample of each group in the stream.  We first want
to note that it is easy to maintain the \emph{xxxxx}-optimal sample of
the stream using two passes and a total of $O(M+r)$ memory: the first
pass computes and save the necessary statistics of each group using
$O(r)$ space.  Then we can use these statistics and the user-given
weight matrix to compute the sample allocation size for each
group. The second pass of the stream is to draw the actual sample of
size $M$ using the offline algorithm from Sections~\ref{xxx}).  

However, the low bound we will present next shows that in general it
is impossible to maintain a CVOPT SRS of size $M$ over a stream in a
single pass using $O(r+M)$ space. The difficulty arises from the fact
that while new stream elements arrive, the sample allocation sizes may
change. However, in general it is impossible to immediately obtain the
actual sample whose allocation size is increased, because, in the
one-pass processing of the stream, old elements are not saved and the
new ones have not arrived yet.

%the picture of the general setting of the streaming scenario


\subsection{A lower bound for streaming group-by sampling}
%\subsection{Single Group-By}
%We consider the lower bound for the \sasg case. 
Given a data stream 
of elements belonging to $r$ groups, and a memory budget of $M$
elements, let $V^*$ denote the optimal $\ell_2$ norm of the CV vector
of a sample of size $M$ drawn by an offline  algorithm that may take multiple
passes over the stream. Suppose $S$ is a stratified random sample of
size $M$ drawn from the stream. Let $V(S)$ denote 
the $\ell_2$ norm of the CV
vector of the sample $S$. Obviously, $V(R) \leq V^*$. 
For any $\alpha > 1$, we say \emph{$S$ is an SRS
with multiplicative error of $\alpha$, if: (1) the sample of each
group is chosen uniformly from all element in the group, and (2) $V(S)
\leq \alpha \cdot V^*$}.

\begin{theorem}
  Any streaming algorithm for maintaining an SRS over a stream with $r$
  groups using a memory of $M$ elements must, in the worst case, result
  in a stratified random sample with a multiplicative error $\Omega(\sqrt{r})$.
\end{theorem}

The idea for the proof is that we construct a stream where each group
share the same (or nearly the same) CV, until a point where one group
receives an element whose value significantly increases the CV of that
group. This is followed by a significantly increased sample allocation
size for that group.  However, the streaming algorithm cannot obtain
such a much larger actual sample for that group using limited memory
space, causing the overall quality of the SRS to be significantly
worse than the optimal one.

\begin{proof}
Consider a stream of $r$ groups named as $1, 2,\ldots, r$. Each group
$i$ takes values from the range $[1, 2)$. Suppose in the current stream, 
each group has $\alpha-1$ copies of $1$ and one copy of
$1+\epsilon$, \ie
$$n_i = \alpha, \ \ \ 
\mu_i=1+\frac{\epsilon}{\alpha}, \ \ \ 
\sigma_i =
\frac{\sqrt{\alpha-1}}{\alpha}\epsilon, \ \ \ 
\frac{\sigma_i}{\mu_i}=\frac{\sqrt{\alpha-1}\epsilon}{\alpha+\epsilon}$$ 
where choose $\alpha\geq 3$ and $\epsilon =\frac{1}{r-1}$.
%
Because of  the memory budget $M$, the sample size of at least one
group (say Group $1$) is no more than $M/r$. Suppose at this moment,
we get a new element of value $2-\epsilon$ belonging to Group $1$. 
Let $n'_1$, $\mu'_1$, and $\sigma'_1$ denote the size, mean, and
standard deviation of all the elements of Group $1$ after receiving this new element, \ie
$$n'_1 = \alpha+1, \ \ \ \mu'_1 = 1 + \frac{1}{\alpha+1}, \ \ \ 
\sigma'_1 = \sqrt{\frac{\epsilon^2+(1-\epsilon)^2 - \frac{1}{\alpha+1}}{\alpha+1}}$$

\begin{eqnarray}
\frac 1 4 \frac{1}{\sqrt{\alpha+1}}
\leq 
\frac{1}{2}\sigma'_1 \leq \frac{\sigma'_1 }{\mu'_1}
\leq \sigma'_1
\leq \frac{1}{\sqrt{\alpha+1}} \label{eqn:1}
\end{eqnarray}

\begin{eqnarray}
\frac 1 {16} \frac{1}{\alpha+1}
\leq \frac{{\sigma'_1}^2 }{{\mu'_1}^2}
\leq \frac{1}{\alpha+1} \label{eqn:4}
\end{eqnarray}
For Groups $2,\ldots, r$, we have:

\begin{eqnarray}
\frac 1 4 \frac{1}{\sqrt{\alpha+1}} \leq 
\frac 1 2 \sum_{i=2}^r\sigma_i  \leq 
\sum_{i=2}^r \frac{\sigma_i}{\mu_i} \leq
\sum_{i=2}^r \sigma_i
\leq \frac{1}{\sqrt{\alpha+1}} \label{eqn:2}
\end{eqnarray}


\begin{eqnarray}
\frac 1 4 \frac{\alpha-1}{\alpha^2(r-1)}
= \frac 1 4 \sum_{i=2}^r\sigma_i^2
\leq 
\sum_{i=2}^r \frac{\sigma^2_i}{\mu_i^2} 
\leq
\sum_{i=2}^r \sigma_i^2
= %(r-1) 
\frac{\alpha-1}{\alpha^2(r-1)}\label{eqn:3}
\end{eqnarray}


Let $V$ denote the $\ell_2$ norm of the vector of CV of all groups
after the streaming algorithm observes the stream of $(r\alpha + 1)$ elements. Let
$V^*$ denote the possible smallest $\ell_2$ norm of the vector of CV of all
groups  with a stratified random sample of size $M$ on this
data. Let $\Delta = \frac{{\sigma'_1}^2}{{n'_1}{\mu'_1}^2}
+\sum_{i=2}^r \frac{{\sigma_i}^2}{{n_i}{\mu_i}^2}$. We observe that
after processing the $r\alpha+1$ elements, the sample size $s_1\leq
M/r+1$. Using this fact and the definition of $V$:  


\begin{eqnarray*}
V^2 &=& 
\frac{{\sigma'_1}^2}{{\mu'_1}^2s_1} 
+ \sum_{i=2}^r \frac{{\sigma_i}^2}{{\mu_i}^2s_i} - \Delta
\geq \frac{{\sigma'_1}^2}{{\mu'_1}^2\frac{M}{r+1}} 
+ \sum_{i=2}^r \frac{{\sigma_i}^2}{{\mu_i}^2\frac{M}{r-1}} - \Delta\\
&\geq&% \frac{r+1}{M}\frac{{\sigma'_1}^2}{{\mu'_1}^2} 
%+ \frac{r-1}{M}\sum_{i=2}^r \frac{{\sigma_i}^2}{{\mu_i}^2} - \Delta\\
%&\geq& \frac{r+1}{M} \frac{1}{16}\frac{1}{\alpha+1}
%+ \frac{r-1}{M} \frac 1 4 \frac{\alpha-1}{\alpha^2(r-1)}- \Delta\\
%&=& 
\frac{r+1}{M} \frac{1}{16}\frac{1}{\alpha+1}
+ \frac{1}{M} \frac 1 4 \frac{\alpha-1}{\alpha^2} - \Delta 
\textrm{\ \
     \ \ \ (Use Ineq.~\ref{eqn:4} and \ref{eqn:3})}\\
\end{eqnarray*}


On the other hand, the optimal (smallest) value $V^*$ of the error metric is
achieved when the sample size of each group is proportional to
$\sigma_i/\mu_i$. Due to Inequalities~\ref{eqn:1}~and~\ref{eqn:2}, the
sample size for Group $1$ is at least $M/5$, while all other groups 
share at least $M/5$ memory space as well. Using these observation
into the definition of $V^*$: 
\begin{eqnarray*}
{V^*}^2 &\leq& 
\frac{{\sigma'_1}^2}{{\mu'_1}^2M/5} 
+ \sum_{i=2}^r \frac{{\sigma_i}^2}{{\mu_i}^2\frac{M}{5(r-1)}} - \Delta\\
&\leq&
\frac 5 M \frac{1}{\alpha+1} 
+ \frac{5}{M}\frac{\alpha-1}{\alpha^2} - \Delta
\textrm{\ \
     \ \ \ (Use Inequalities~\ref{eqn:4} and \ref{eqn:3})}\\
\end{eqnarray*}

Because $\Delta > 0$ and $M > r$, 

$$
\frac{V}{V^*} = \Omega(\sqrt{r})
$$
\end{proof}

\todo{We want to note that this lower bound is tight (up to constant
  factors), because the uniform allocation for SASG yields an error
  that is within an $O(\sqrt{r})$ multiplicative error. This claim as
  well as the similar claim in the EDBT submission
  needs double check, because of the existence of the $\Delta$ term in
  the above proof.}


\subsection{A locally cv-optimal stream sampling method for group-by queries}
We now present a streaming algorithm that can maintain a stratified random
sample over the stream of table tuples in a \emph{locally} \varopt
manner. The algorithm supports mini-batch based processing, and the
size of each mini batch received by the stream sampler is allowed to
be dynamically changing over the progress of the stream.  
When the mini batch size is always one, the sampler
is a pure streaming algorithm, whereas in the other extreme case where
the mini batch size is equal to the entire stream size, the streaming
sampler automatically reduces to the offline \varopt samplers
(Section~\ref{xxx}). 

\subsubsection{The maintenance of uniformity of the sample}
The first issue is the maintenance of the uniformity of each sample
$S_i$ drawn from the elements belonging to group $i$ that have been
received so far. We use the \emph{key} based
idea for maintaining a uniform random sample. When a new stream
element arrives, the stream sampler assign the element a key randomly drawn from
$(0,1)$. Each sample $S_i$ always only keep those elements 
whose key values are among the smallest. Specifically, for each sample
$S_i$, let $d_i$ always record the value of the smallest key that have
been discarded from sample $S_i$. For each element in the newly
received mini batch, if the element's key is less
than or equal to $d_i$, the new element is inserted to sample $S_i$;
otherwise, it will be discarded right away. After the processing of
the mini batch of elements, the size of the SRS may exceed the memory
budget $M$. So next, we need to address the question on what elements
need to be evicted from the SRS such that the memory budget $M$ is
maintaned and the increase of the $\ell_2$ norm of the CV vector of
the sample is minimized. We first abstract the offline samplers in the
previous sections into a common optimization problem. 


\subsubsection{The common optimization problem that abstracts the offline VCOPT
  samplers.} 
The problem and solution for VCOPT sampling for  \sasg, \samg, \masg,
and \mamg queries that we have studied in the previous sections can be
abstracted as the following optimization problem: We are given a data set of
$k$ groups, a memory budget  of $M$ elements, and a set of group-by queries.
Let $f(i)$ be a positive valued function of group $i$. 
Once the data set and
the queries are given, each $f(i)$ becomes a positive constant. 
\begin{itemize}
\item \sasg:   $f(i) = ....$ 
\item   \samg: $f(i) = ....$
\item  \masg:  $f(i) = ....$ 
\item  \mamg: $f(i) = ....$ 
\end{itemize}
We want to
minimize 
$$F = \sum_{i=1}^k \frac{f^2(i)}{M_i},$$ 
subject to the constratint
$$\sum_{i=1}^k M_i = M.$$ 
The solution to this optimization problem is
each  
$$M_i = M \frac{f(i)}{\sum_{j=1}^k f(j)}.$$ 
We call $M_i$ the VCOPT sample allocation size for group $i$ for the
given set of group-by queries and under
the memory budget $M$. 


\subsubsection{Maintaining the memory budget via \varopt sample size reduction}
After all elements in the new mini batch are processed, the sample
size may exceed the memory budget $M$ due to the possible insertion of
new elements into the SRS. 
Now the question we need to address is: \emph{How to reduce the
  current SRS size back to $M$, such that every sample $S_i$ still
maintains its uniformity and the increase of the value of  the objective function
is minimized?} 
%
More precisely, let $S' = S_1'\cup \ldots \cup S_k'$ be the SRS of the current data stream
of $k$ groups, where $S_i'$ is the sample of group $i$ and has size $s_i'$. 
Say the size of $S'$, $\sum_{i=1}^k s'_i$, is   $M'= M +
\beta$. Our goal is to evict $\beta$ elements from $S'$
such that the smaple of each group still maintaines its unifomilyt and
the increase of the value of $F$ is minimized. 

We say sample $S'_i$ is \emph{oversized} if $s'_i > M_i$; otherwise,
$S'_i$ is \emph{not oversize}.  The next Lemma says the all the
$\beta$ evictions must be made from the oversize samples such that the
increase of the objective function $F$
is minimized.


\begin{lemma}
\label{lem:evict}
Suppose that $E$ is the set of $\beta$  elements to be evict from the
$S'$ such that the increase of $F$ is 
minimized. Then, each element of $E$ must be from an oversized
sample under the memory budget $M$. 
\end{lemma}

\begin{proof}
 We use the proof by contradiction.  Suppose there is an element $e\in
 E$ is evicted from a group $\alpha$ which is not oversized. Because
 the sequence of eviction does not affect the value of the objective
 function after all $\beta$ evictions have happened, suppose $e$ is
 evicted at the moment $t$ that is right after all other $\beta-1$ evictions have happened. Let
 $s_\alpha$ denote the size of sample $S_\alpha$ right
 after the $\beta-1$ evictions. After the eviction of $e$, the change
 of the value of the objective function $F$ is: 
$$
   \Delta  = \frac{f^2(\alpha)}{s_\alpha(s_\alpha-1)} = 
\left(\frac{\sum_{i=1}^kf(i)}{M} \right)^2 
\frac{M_\alpha^2}{s_\alpha(s_\alpha-1)} > \left(\frac{\sum_{i=1}^kf(i)}{M} \right)^2.
$$
%where $M_\alpha = M\frac{f(\alpha)}{\sum_{i=1}^kf(i)}$. 
The last
inequality is due to the fact that $S_\alpha$ is not oversized, \ie
$s_\alpha \leq M_\alpha$.

Suppose at time $t$,
we choose to
evict an element $e'$ from another sample $S_{\alpha'}$ that is
oversized. Note that such an oversized sample must be existing, because
at time $t$ the size of the SRS size is $M+1$. After evicting $e'$ from
$S_{\alpha'}$, the increase of the vluae of the objective function $F$
is: 
$$
   \Delta' = \frac{f^2({\alpha'})}{s_{\alpha'}(s_{\alpha'}-1)} = 
\left(\frac{\sum_{i=1}^kf(i)}{M} \right)^2 
\frac{M_{\alpha'}^2}{s_{\alpha'}(s_{\alpha'}-1)}
< \left(\frac{\sum_{i=1}^kf(i)}{M} \right)^2.
 $$
%where $M_{\alpha'} = M\frac{f({\alpha'})}{\sum_{i=1}^kf(i)}$. 
The last
inequality is due to the fact that $S_{\alpha'}$ is oversized, \ie
$s_{\alpha'} > M_{\alpha'}$.

Because $\Delta' < \Delta$, we should evict $e'$ instead of $e$ in
order to achieve a smaller increase of the value of the objective
function $F$. This is a contradition to the assumption that the eviction
of $e$ leads to the minimum increase of the value of $F$, 
so the lemma is proved.  
\end{proof}

Among the samples $S'_1, \ldots, S'_k$, let $\mathcal{O}$ denote the
set of oversized samples, $\mathcal{U}$ denote the set of samples that
are not oversized.  Lemma~\ref{lem:evict} tells us that all samples
from $\mathcal{U}$ will not need to change in the eviction of $\beta$
elements, and we only need to evict the $\beta$ elements from the
samples from $\mathcal{O}$. The next lemma says the eviction of
$\beta$ elements can indeed be recursively solved among the samples in
$\mathcal{O}$ under the new memory budget
$M- \sum_{i\in \mathcal{U} s_i}$. The base case is where every sample
under consideration is oversized. In that base, we can evict the
$\beta$ elements by  simply setting each sample size to be its VCOPT
optimal allocation size under the memory budget being considered. 


\begin{lemma}
  \label{lem:recur}
The $F$-optimal eviction of $\beta$ elements from $S'$ requires the
$F$-optimal eviction of $\beta$ elements from $\mathcal{O}$.
\end{lemma}

\begin{proof}
After the eviction of $\beta$ elements, 
let $s_1, \ldots, s_k$ denote the sample size of each group. 
The $F$-optimal eviction of $\beta$ elements requires to minimize
\begin{eqnarray}
\label{eqn:5}
\sum_{i=1}^k \frac{f^2(i)}{s_i} -\sum_{i=1}^k \frac{f^2(i)}{s'_i}
\end{eqnarray}
By Lemma~\ref{lem:evict}, we know those samples in $\mathcal{U}$ will
not change. So minimizing Formula~\ref{eqn:5} is equivalent to
minimizing 
\begin{eqnarray}
\label{eqn:6}
\sum_{i\in \mathcal{O}}\frac{f^2(i)}{s_i} -\sum_{i\in \mathcal{O}} \frac{f^2(i)}{s'_i}
\end{eqnarray}
under the new memory budget $M-\sum_{i\in \mathcal{U}}s_i'$.
\end{proof}


\begin{observation}
  In the case every sample is oversized under the target memory budget
  $M$, \ie $\mathcal{O} \ emptyset$, the $F$-optmail eviction of
  $\beta$ elements is simply setting each sample size $s_i = M_i$
  under the memroy budget $M$.
\end{observation}

\todo{Give the pseudocode of the streaming sampler for
group-by queries. }


\begin{theorem}
\todo{recursion based imp}  
\end{theorem}


\begin{theorem}
\todo{fast iteration based imp}  
\end{theorem}







\todo{Sliding Window needed ? }




%focus on the weighted, multiple aggregate, single group-by

%the batch based processing

%sliding window stuff





==> workload.tex <==
%--------------------------------
\section{Using A Query Workload}
\label{sec:workload}
%--------------------------------
How can one use (partial) knowledge of the query workload to improve sampling? A query workload is a set of queries or a probability distribution of queries that can be expected to be posed. A query workload can be either collected from historical query logs or created by users based on their experience. In our case, we can profitably use information about certain aspects of the query workload. 

Specifically, in the presence of information about the aggregation columns and the group-by attributes, such as the probability distribution of the aggregation column and of the group-by attributes, we show how to construct a sample that is optimized for this workload. We focus on the case of multiple aggregations, multiple group-by (MAMG), since the other cases, such as SASG and MASG are special cases.

Our approach is to reduce the handling of a query workload to the case of weighted optimization of group-by queries. Given a query workload, we derive the different combination of the pairs of group-by attributes and aggregation columns. For each such combination, we assign a frequency, depending on the number of times this combination occurs, across all queries. We then use this as a weight in our weighted optimization framework. For example, if a workload has the following queries


\remove{
For instance,
the distribution of queries on different aggregate columns, the
distribution of different combinations of group-by attributeds,
etc. Given a query workload, the system designer is empowered by
knowing well about future that helps optimize the design of the
system. The basic idea in query workload-driven design for approximate
query processing is to give a bias for better accuracy guarantee to
those queries of higher frequency and thus of more importance. In this
section, we explain a well intuitive mechanism that preprocesses a
given query workload and produces a parameterization for the biasness
that favors queries of more importance, for the MAMG case. The
query workload preprocessing for other cases (SASG, MASG, SAMG) will
only be a special case of the mechasim for MAMG workload
preprocessing. The preprocessing of the workload produces as output
the value of the weights that we used in our framework for optimized
random sampling for group-by queries. 
}

Each group-by query in the given query workload stratifies each
aggregated column into a collection of disjoint subcolumns. The number
of subcolumns is equal to the number of groups. We call
each subcolumn as an \emph{entity}. For example,
suppose the university has 10 majors, then 
%a group-by query
%\texttt{SELECT major, AVG(gpa) FROM student GROUP BY major} stratifies
%the \texttt{gpa} column into 10 subcolumns and the average GPA of each
%subcolumn is an entity.  Similarly, 
a group-by query \texttt{SELECT major,
  AVG(gpa), AVG(age) FROM student GROUP BY major} 
stratifies both the \texttt{gpa}  the \texttt{age} columns into 10
subcolumns, 
 and therefore there are a total of 20
entities of interest induced by this group-by query.
%produces $20$
%entities. 
Let $\mathcal{W}$ denote the collection of all entities induced 
by a given query workload. Note that $\mathcal{W}$ is a multiset
because a certain entity may appear in multiple queries in the
workload. 
Our goal is to let the designer to decide the relative importance
(weight) of each of these entities. 
For example, if the designer wants to  offer an equal level of accuracy guarantee to the
aggregation of each of these
entities and want to minimize the $\ell_2$ norm of the CVs of their
estimation: 

\begin{eqnarray}
\sum_{e\in \mathcal{W}} (\cv{\widehat{agg}(e)})^2
= \sum_{e\in \mathcal{D}} f_e \cdot (\cv{\widehat{agg}(e)})^2
\label{eqn:workload}
\end{eqnarray}
where $\widehat{agg}(e)$ denote the estimate of the aggregate function
value of the entity $e$ obtained from
using the sample, $\mathcal{D}$ denote the set of distinct entities
from $\mathcal{W}$, $f_e$ represents the frequency of an entity $e$.
By comparing the above quantity~\ref{eqn:workload} that we want to
minimize  with the definition of the weighted group (Equation~\ref{eq:weight}), 
we can set the weight value $w_e$ of each distinct $e$ to be
proportional to $f_e$, e.g., $w_e = \frac{f_e}{\sum_{\alpha\in\mathcal{E}}f_\alpha}$, our optimized
random sampling framework for group-by queries can take as input a
given query workload to produce bias toward better accuracy guarantee
for entities that are queried more often.

We also want to note that users do have their own discretion to decide the query workload preprocessing mechanism based on the actual needs in their application. For example, they can set each $w_e$ to be proportional to $\sqrt{f_e}$, if it is more appropriate for their systems. Or, any particular $w_e$ can be manually tuned up or down based on the needs from applications.  However, the change of the internal mechanism for workload preprocessing is transparent to and thus does not affect the sampling framework that we presented in the previous sections, making our sampling strategy to be flexible enough to have an add-on workload preprocessor.








